Efficient and Privacy-Preserving Infection Control System for Covid-19-Like Pandemics using Blockchain

Contact tracing is a very effective way to control the COVID-19-like pandemics. It aims to identify individuals who closely contacted an infected person during the incubation period of the virus and notify them to quarantine. However, the existing systems suffer from privacy, security, and efficiency issues. To address these limitations, in this paper, we propose an efficient and privacy-preserving Blockchain-based infection control system. Instead of depending on a single authority to run the system, a group of health authorities, that form a consortium Blockchain, run our system. Using Blockchain technology not only secures our system against single point of failure and denial of service attacks, but also brings transparency because all transactions can be validated by different parties. Although contact tracing is important, it is not enough to effectively control an infection. Thus, unlike most of the existing systems that focus only on contact tracing, our system consists of three integrated subsystems, including contact tracing, public places access control, and safe-places recommendation. The access control subsystem prevents infected people from visiting public places to prevent spreading the virus, and the recommendation subsystem categorizes zones based on the infection level so that people can avoid visiting contaminated zones. Our analysis demonstrates that our system is secure and preserves the privacy of the users against identification, social graph disclosure, and tracking attacks, while thwarting false reporting (or panic) attacks. Moreover, our extensive performance evaluations demonstrate the scalability of our system (which is desirable in pandemics) due to its low communication, computation, and storage overheads.

==> Files/SystemModels.tex <==

\section{System and Threat Models}\label{models}
In this section, we discuss the system and threat models considered in this paper.
\subsection{System Model}
Fig. \ref{overview} shows the different entities in our net-metering system and the interactions between them. At the customer side, there are solar panels installed on the rooftop of the customer's house. These solar panels convert the energy collected from the sun to  direct current (DC) electricity which cannot be used directly to power the house's appliances or injected to the grid. Therefore, an inverter is used to convert the DC electricity to alternating current (AC) electricity. Then, the AC electricity flows from the inverter to the main service panel that controls feeding the electricity to the house's appliances. 
In the net-metering system, the customer's solar generation system is connected to the utility's power grid as shown in Fig. \ref{overview} so that the excess power generated can be injected directly to the grid through the net meter, and thus, the customer does not need to purchase an expensive solar battery. On the other hand, if the generated power is insufficient, the customer can satisfy his consumption needs by drawing electricity from the power grid through the net meter. Thus, the net meter acts as an interface between the customer and the utility, and it is a bidirectional meter that allows the electricity flow in either direction. 

The net meter periodically records readings, which represent the difference between the power consumed by the house appliances and the power generated by the solar panels.
Therefore, the reading is positive if the consumed power is more than the generated power, the reading is negative if the generated power is more than the consumed power, and the reading is zero if the consumed power is similar to the generated power.
These fine-grained readings are communicated to the utility's control center through the AMI network via wired communications such as power line communication or wireless communication such as cellular communication \cite{wang2011survey}. These readings are used by the utility for billing purposes and for demand side management (i.e, achieving a balance between the energy demand and supply).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Threat Model}
Given the high installation costs of the solar generation system, customers may be keen to get as high profits as they can from the system even by illegal ways to shorten the time taken to compensate the paid costs. In doing so, malicious customers may launch false-reading attacks by compromising their net meters to report false readings to the utility to achieve financial gains illegally. Specifically, malicious customers can report lower readings when the consumed power is more than the generated power (in case of positive readings) and report higher readings when the generated power is more than the consumed power (in case of negative readings). 

SMs can be compromised to report false readings by programming a malicious firmware and installing it in the SM that is accessible through the ANSI optical port \cite{ismail2018}. This port is usually secured via weak passwords and there are some tools, such as Terminator, that are used to launch brute force attack to guess the passwords and gain access to the SM \cite{ismail2018}.
Moreover, recent studies have shown that the AMI communication networks have vulnerabilities, which can be exploited by malicious customers to launch the false-reading attacks \cite{8039510}.
The false reported readings not only cause financial losses to the utility but also can result in wrong decisions regarding energy management. Thus, in this paper, we propose a deep learning-based detector to analyze the readings reported by the customers' net meters to detect the false-reading attacks.


==> Files/bio.tex <==
\section*{Biographies}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{}}]{Seham A. Alansari }
received a B.Sc. degree in Computer Science from Umm Al-Qura University, Mecca, Saudi Arabia, in 2015. She is currently pursuing her M.S. degree in Computer Science and Engineering at Umm Al-Qura University, Mecca, Saudi Arabia. She received a Higher diploma degree in Education from Umm Al-Qura University, Mecca, Saudi Arabia, in 2016. From 2015 to 2017, she worked as a Research Assistant in the Department of Computer Science at Umm Al-Qura University, Mecca, Saudi Arabia. Her research interests include Blockchain, security, and privacy.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Files/Pics/MahmoudBadr.jpg}}]{Mahmoud M. Badr}
is currently a Graduate Research Assistant in the Department of Electrical \& Computer Engineering, Tennessee Tech. University, TN, USA and pursuing his Ph.D. degree in the same department. He is also holding the position of a Lecturer Assistant at the Faculty of Engineering at Shoubra, Benha University, Egypt.
He received the B.S. and M.S. degrees in Electrical Engineering from Benha University, Cairo, Egypt in 2013 and 2018, respectively.
His research interests include blockchain, cryptography, 5G networks, network security, and smart grids.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Files/Pics/mohamed_mahmoud.jpg}}]{Dr. Mohamed M. E. A. Mahmoud}
	received PhD degree from the University of Waterloo in April 2011. From May 2011 to May 2012, he worked as a postdoctoral fellow in the Broadband Communications Research group - University of Waterloo. From August 2012 to July 2013, he worked as a visiting scholar in University of Waterloo, and a postdoctoral fellow in Ryerson University. Currently, Dr. Mahmoud is an associate professor in Department Electrical and Computer Engineering, Tennessee Tech University, USA. The research interests of Dr. Mahmoud include security and privacy preserving schemes for smart grid communication network, mobile ad hoc network, sensor network, and delay-tolerant network. Dr. Mahmoud has received NSERC-PDF award. He won the Best Paper Award from IEEE International Conference on Communications (ICC'09), Dresden, Germany, 2009. Dr. Mahmoud is the author for more than twenty three papers published in major IEEE conferences and journals, such as INFOCOM conference and IEEE Transactions on Vehicular Technology, Mobile Computing, and Parallel and Distributed Systems. He serves as an Associate Editor in Springer journal of peer-to-peer networking and applications. He served as a technical program committee member for several IEEE conferences and as a reviewer for several journals and conferences such as IEEE Transactions on Vehicular Technology, IEEE Transactions on Parallel and Distributed Systems, and the journal of Peer-to-Peer Networking.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Files/Pics/Waleed.jpg}}]{Dr. Waleed Alasmary} (SM'19) received the B.Sc. degree (Hons.) in computer engineering from Umm Al-Qura University, Saudi Arabia, in 2005, the M.A.Sc. degree in electrical and computer engineering from the University of Waterloo, Canada, in 2010, and the Ph.D. degree in electrical and computer engineering from the University of Toronto, Toronto, Canada, in 2015. During his Ph.D. degree, he was a Visiting Research Scholar with Network Research Laboratory, UCLA, in 2014. He was a Fulbright Visiting Scholar with CSAIL Laboratory, MIT, from 2016 to 2017. He subsequently joined the College of Computer and Information Systems, Umm Al-Qura University, as an Assistant Professor of computer engineering, where he currently holds an Associate Professor position. His ``Mobility impact on the IEEE 802.11p'' article is among the most cited Ad Hoc Networks journal articles list from 2016-2018. He is currently an Associate Editor for the Array journal.
\end{IEEEbiography}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

